Contribution to Blocker and Interdiction optimization problems in networks

This manuscript describes the notions of blocker and interdiction applied to well-known optimization problems. The main interest of these two concepts is the capability to analyze the existence of a combinatorial structure after some modifications. We focus on graph modification, like removing vertices or links in a network. In the interdiction version, we have a budget for modification to reduce as much as possible the size of a given combinatorial structure. Whereas, for the blocker version, we minimize the number of modifications such that the network does not contain a given combinatorial structure. Blocker and interdiction problems have some similarities and can be applied to well-known optimization problems. We consider matching, connectivity, shortest path, max flow, and clique problems. For these problems, we analyze either the blocker version or the interdiction one. Applying the concept of blocker or interdiction to well-known optimization problems can change their complexities. Some optimization problems become harder when one of these two notions is applied. For this reason, we propose some complexity analysis to show when an optimization problem, or the associated decision problem, becomes harder. Another fundamental aspect developed in the manuscript is the use of exact methods to tackle these optimization problems. The main way to solve these problems is to use integer linear programming to model them. An interesting aspect of integer linear programming is the possibility to analyze theoretically the strength of these models, using cutting planes. For most of the problems studied in this manuscript, a polyhedral analysis is performed to prove the strength of inequalities or describe new families of inequalities. The exact algorithms proposed are based on Branch-and-Cut or Branch-and-Price algorithm, where dedicated separation and pricing algorithms are proposed.

==> Acronymes.tex <==
%!TEX root = Manuscrit.tex

\chapter*{Liste d'abréviations}
\mtcaddchapter[Liste d'abréviations]

% Define here acronyms used in the manuscript. Copy paster the example for each new acromnym you would like to use

\begin{acronym}
\renewcommand{\\}{}
\acro{DTI}{Diffusion Tensor Imaging}
\end{acronym}


==> chapters/CV.tex <==
\chapter{Curriculum Vit\ae}

\section*{Sébastien Martin}
\paragraph{Principal Research Engineer at Huawei} ~\\
Tel: +33.6.10.71.12.21\\
Mail: sebastien.martin@huawei.com\\
Website: http://martin.site.free.fr/index.php\\

\section{Cursus and professional experiences}
\begin{itemize}
    \item 2018 -- now: Principal Research Engineer at Huawei
    \item 2012 -- 2018: Assistant professor at LCOMS laboratory of University of Lorraine
    \item 2007 -- 2012: PhD in Computer Science and Combinatorial Optimization and Teaching Assistant, Université Paris Dauphine, Paris.
    \item 2005 -- 2007: Masters degrees in Computer Science, Artificial Intelligence, Learning and Decision, Université Pierre et Marie Curie, Paris
\end{itemize}

\section{PhD Supervisions}

\paragraph{Isma Bentoumi} (2019-)\\
{\it Optimization method for the multi-commodity flow blocker problem.}\\
Co-supervised: Fabio Furini (33\%), Ridha Mahjoub (33\%), Sébastien Martin (33\%)\\

\paragraph{Sarah Minich} (2017-2022)\\
{\it Approximation algorithms for solving some pagination problems.}\\
Co-supervised: Imed Kacem (33\%), Aristide Grange (33\%), Sébastien Martin (33\%)\\

\paragraph{Youcef Magnouche} (2013-2017)\\
{\it The multi-terminal vertex separator problem: Complexity, Polyhedra and Algorithms.}\\
Co-supervised: Denis Cornaz (33\%), Ridha Mahjoub (33\%), Sébastien Martin (33\%)\\

\paragraph{Mohammed Albarra Hassan Abdeljabbar Hassan} (2013-2016)\\
{\it Robust scheduling problem for cloud computing}\\
Co-supervised: Imed Kacem(50\%), Sébastien Martin (50\%)\\

\paragraph{Mohamed Ould} (2011-2014)\\
{\it Combinatorial optimization and knowledge on companies}\\
Co-supervised: Ridha Mahjoub (50\%), Sébastien Martin (50\%)\\



\section{Master Student supervisions}
Full or partial supervision.\\
\begin{itemize}
    \item Corentin Clavier (2021) {\it OSPF decomposition area and combinatorial optimization}
    \item Corentin Juvigny(2020) {\it On the shortest path problem with node inclusion} 
    \item Alexandre Schulz(2019) {\it Machine learning applied to shortest path problems} 
    \item Mathieu Kintzinger(2015) {\it Robust nurse assignment problem with priority} 
    \item Karine Laurent(2015) {\it On the knapsack problem with overlapping object} 
    \item Xin Wang(2015) {\it Heuristic and meta-heuristic for the $k$-separator problem} 
    \item Zheng Mengli(2014) {\it Column generation algorithm for the robust nurse assignment problem} 
    \item Xiaotong Jiao(2013) {\it Uni-dimensional cutting problem} 
    \item Ali Taleb(2012) {\it A branch-and-bound algorithm for a scheduling problem} 
\end{itemize}
    
\section{International journals}
The authors are given in alphabetic order for the references with a $*$. 
\begin{enumerate}
    \item V. Angilella, F. Krasniqi, P. Medagliani, S. Martin, J. Leguay, R. Shoushou, L. Xuan. {\it High capacity and Resilient Large-scale Deterministic IP Networks}. ournal of Network and Systems Management. To appear 2022.
    \item S. Martin, Y. Magnouche, C. Juvigny, J. Leguay. {\it Constrained shortest path tour problem: Branch-and-Price algorithm}. Elsevier Journal on Computers and Operations Research. April 2022.
    \item J. Krolikowski, S. Martin, P. Medagliani, J. Leguay., S. Chen, X. Chang and X. Geng. {\it Joint Routing and Scheduling for Large-Scale Deterministic IP Networks}. Elsevier Computer Communications. October 2020.
    \item* D. Cornaz, Y. Magnouche, A. R. Mahjoub and S. Martin. {\it The multi-terminal vertex separator problem : Branch-and-Cut-and-Price}. Discrete Applied Mathematics. 2020
    \item* Y. Magnouche and S. Martin. {\it Most Vital Vertices for the Shortest s-t Path Problem : Complexity and Branch-and-Cut algorithm}. Optimization Letters. 2020
    \item* P. Laroche, F. Marchetti, S. Martin, A. Nagih, Z. Róka. {\it Multiple Bipartite Complete Matching Vertex Blocker Problem: Complexity, polyhedral analysis and Branch-and-Cut}. Discrete Optimization, Available online 6 August 2019, 100551
    \item* F. Furini, I. Ljubić, S. Martin, P. San Segundo. {\it The Maximum Clique Interdiction Problem}, European Journal of Operational Research. Volume 277, Issue 1, 16 August 2019, Pages 112-127.
    \item* D. Cornaz, Y. Magnouche, A. R. Mahjoub and S. Martin. {\it The multi-terminal vertex separator problem : Polyhedral analysis and Branch-and-Cut}. Discrete Applied Mathematics. 2019, 256 (1).
    \item* D. Cornaz, F. Furini, M. Lacroix, R. Mahjoub, E. Malaguti, S. Martin. {\it The Vertex $k$-cut Problem}.Discrete Optimization.Volume 31, February 2019, Pages 8-28.
    \item* M. A. Hassan, I. Kacem, S. Martin, I. M. Osman. {\it On the m-clique free interval subgraphs polytope: polyhedral analysis and applications}. Journal of Combinatorial Optimization, DOI: 10.1007/s10878-018-0291-9 (2018).
    \item* A. Grange, I. Kacem, S. Martin. {\it Algorithms for the Bin Packing Problem with Overlapping Items}. Computers \& Industrial Engineering 115: 331-341 (2018).
    \item* L. Alfandari, T. Davidovi, F. Furini, I. Ljubic, V. Maras, S. Martin. {\it Tighter MIP formulations for Barge Container Ship Routing}. Omega https://doi.org/10.1016/\- j.omega.2017.12.002 (2017).
    \item* M. A. Hassan, I. Kacem, S. Martin, I. M. Osman. {\it Genetic Algorithms for Job Scheduling in Cloud Computing}. Studies in Informatics and Control, ISSN 1220-1766, vol. 24 (4), pp. 387-400, 2015.
    \item* M. Lacroix, A. R. Mahjoub, S. Martin et C. Picouleau. {\it On the NP-Completeness of the Perfect Matching Free Subgraph Problem}. Theoretical Computer Science, Vol. 423, pages 25-29 (2012).
    \item* M. Lacroix, A. R. Mahjoub et S. Martin. {\it Combinatorial Optimization Model and MIP formulation for the Structural Analysis of Conditional Differential-Algebraic Systems}. Computers \& Industrial Engineering 61 (2011), pp. 422-429.
\end{enumerate}

\section{International conferences}
\begin{enumerate}
\item T. A. Q. Pham, S. Martin, J. Leguay, Xu Gong, Xu Huiying. Intent-Based Routing Policy Optimization in SD-WAN. IEEE ICC 2022. Seoul, South Korea. May 2022.
\item Y. Magnouche, S. Martin, J. Leguay, F. De-Pellegrini, R. El-Azouzi, C. Richier. Branch-and-Benders-Cut Algorithm for the Weighted Coflow Completion Time Minimization Problem. INOC 2022. Aachen, Germany. March 2022.
\item S. Martin, P. Medagliani, J. Leguay. Network Slicing for Deterministic Latency. CNSM HiPNet 2021. Izmir, Turkey. October 2021.
\item  B. Liu, S. Ren, C. Wang, V. Angillela, P. Medagliani, S. Martin, J. Leguay. Towards Large-Scale Deterministic IP Networks. IFIP Networking 2021. Helsinki, Finland. June 2021.
\item* A. Grange, I. Kacem, S. Martin, S. Minich. Approximate solutions for a special pagination problem with 2 symbols per tile. ICNSC 2021.
\item* S. Chen, J. Leguay, S. Martin and P. Medagliani. Load Balancing for Deterministic Networks. TENSOR (IFIP Networking Workshop). Paris, France. June 2020.
\item* N. Huin, J. Leguay, S. Martin, P. Medagliani, S. Cai. Routing and Slot Allocation in 5G Hard Slicing. INOC 2019.
\item* A. Grange, I. Kacem, S. Martin, S. Minich. Fully polynomial-time approximation scheme for the pagination problem. Proceedings of International Conference on Computers and Industrial Engineering, CIE 2019.
\item* F. Furini, E. Malaguti, S. Martin and I. C. Ternier. ILP Models and Column Generation for the Minimum Sum Coloring Problem. à paraître INOC 2017
\item* P. Laroche, F. Marchetti, S. Martin et Z. Roka. " Bipartite Complete Matching Vertex Interdiction Problem with Incompatibility Constraints: Complexity and Heuristics ". IEEE International Conference Control, Decision and Information Technologies Proceedings CODIT 2017, à paraître (2017)
\item* M. Hassan, I. Kacem, S. Martin and I. M.Osman. " Mathematical Formulation for Open Shop Scheduling Problem ". IEEE International Conference Control, Decision and Information Technologies Proceedings CODIT 2017, à paraître (2017)
\item* M. Becker, N. Ginoux, S. Martin and Zs. Roka. Optimization of Tire Noise by Solving an Integer Linear Program (ILP) 2016 IEEE International Conference on Systems, Man, and Cybernetics (SMC2016), 9-12 Octobre 2016, Budapest (Hongrie)
\item* Y. Magnouche and S. Martin. "The Multi-terminal vertex separator problem: Polytope characterization and TDI-ness". Proceedings ISCO 2016, LNCS à paraître (2016)
\item* M. Hassan, I. Kacem, S. Martin and I. M.Osman. "Unrelated Parallel Machine Scheduling Problem With precedence Constraints: Polyhedral Analysis and Branch-and-Cut". Proceedings ISCO 2016, LNCS à paraître (2016)
\item* Y. Magnouche, A. R. Mahjoub and S. Martin. "The Multi-terminal vertex separator problem: Extended formulations and Branch-and-Cut-and-Price". Proceedings CODIT 2016, à paraître (2016)
\item* M. Hassan, I. Kacem, S. Martin and I. M.Osman. "Valid Inequalities for Unrelated Parallel Machines Scheduling with Precedence Constraints". Proceedings CODIT 2016, à paraître (2016)
\item* D. Cornaz, Y. Magnouche, A. R. Mahjoub and S. Martin. " The multi-terminal vertex separator problem: polyhedral analysis and branch-and-cut ". Proceedings of 45th International Conference on Computers \& Industrial Engineering (CIE45), ISBN:9781510817456 pages 857-864 (2015).
\item* M. Hassan Abdel-Jabbar, I. Kacem, S. Martin and I. M. Osman. " Mathematical Formulations for the Unrelated Parallel Machines with Precedence Constraints ". Proceedings of 45th International Conference on Computers \& Industrial Engineering (CIE45), ISBN:9781510817456 pages 1005-1012 (2015).
\item* P. Laroche, F. Marchetti, S. Martin, Z. Roka and M. Zheng. " Complexity and Heuristics for Multi Bipartite Complete Matching Vertex Interdiction Problem: Application to Robust Nurse Assignment ". Proceedings of 45th International Conference on Computers \& Industrial Engineering (CIE45), ISBN:9781510817456 pages 1294-1301 (2015).
\item* A. Grange, I. Kacem, K. Laurent, S. Martin. " On the knapsack problem under merging objects' constraints ". Proceedings of 45th International Conference on Computers \& Industrial Engineering (CIE45), ISBN:9781510817456 pages 1359-1366 (2015).
\item* P. Laroche, F. Marchetti, S. Martin et Z. Roka. " Bipartite Complete Matching Vertex Interdiction Problem: Application to Robust Nurse Assignment ". IEEE International Conference Control, Decision and Information Technologies (CoDIT'14) pages 182-187, (2014).
\item* D. Cornaz, F. Furini, M. Lacroix, E. Malaguti, A. R. Mahjoub et S. Martin. “Mathematical formulations for the Balanced Vertex k-Separator Problem”. IEEE International Conference Control, Decision and Information Technologies (CoDIT'14) pages 176-181, (2014).
\item* M. A. Hassan Abdel-Jabbar, I. Kacem et S. Martin. " Unrelated parallel machines with precedence constraints: Application to cloud computing ". IEEE CLOUDNET 2014pages 438-442, (2014).
\item* M. Lacroix, A. R. Mahjoub et S. Martin. " Polyhedral Analysis and Branch-and-Cut for the Structural Analysis Problem ". Lecture Notes on Computer Science (International Symposium of Combinatorial Optimization (ISCO) 2012), (2012).
\item* M. Lacroix, A. R. Mahjoub et S. Martin. " Structural analysis for Differential-Algebraic Systems: Complexity, Formulation and Facets ". Proceedings ISCO 2010, Electronic Notes in Discrete Mathematics 36, pages 1073-1080.
\item* M. Lacroix, A. R. Mahjoub et S. Martin. "Structural analysis in Differential-Algebraic Systems and Combinatorial Optimization". Proceedings of 39th International Conference on Computers \& Industrial Engineering (CIE39), pages 331-337 (2009). (This publication won the best student paper award)
\item P. Fouilhoux, S. Martin et M. Coupechoux "Combinatorial problems and integer formulations in wireless mesh network design". NCP07 (International Conference on Nonconvex Programming) (2007).
\end{enumerate}

\section{Patents}
\begin{enumerate}
\item Apparatus and method for distributed load balancing in IP routing (2021)
\item Intent-based smart policy-routing (2021)
\item Apparatus and methods for delay-constrained redundant paths in IP routing (2021)
\item Apparatus and methods for virtual topologies in IP routing (2020)
\item Fast Failover for Path Degradation (2020)
\item A load balancing system for deterministic networks (2020)
\item Apparatus and Methods for Protected Load Balancing (2020)
\item Apparatus and Method for coflow tracking to schedule traffic (2020)
\item Resource reconfiguration for Deterministic Networking (2019)
\end{enumerate}

\section{Responsibilities}
\begin{itemize}
    \item Management of the PRC DataCom patent review board (2022 -- )
    \item Member of the PRC DataCom patent review board (2020 -- )
    \item Member of the LCOMS council (2013 -- 2018)
    \item Management of LCOMS DOP seminar (2013 -- 2018)
    \item Head of computer science departement of Metz IUT (2016 -- 2018)
    \item Member of the IUT of Metz council (2012 -- 2018)
\end{itemize}

\section{Projects Involvement}
Management of projects with $^*$ and participation for the other ones. 
\begin{itemize}
\item Huawei project 2022$^*$: MCF solver .
\item Huawei project 2019: Co-flow scheduling algorithm.
\item PEPS 2018 project$^*$: Aide à la décision pour renforcer la robustesse des plannings.
\item Regional 2016 project$^*$: Gestion du personnel paramédical.
\item PHC PAVLE SAVIC 2016: The development of hybrid heuristics for combinatorial optimization.
\item European 2016: Empowering Young Researchers (EYE).
\item PGMO 2015 project: Efficient exact algorithms for Graph Partitioning Problems.
\item PGMO 2014 project: Efficient exact algorithms for Graph Partitioning Problems.
\item ANR 2006 project: Parallel numerical Algorithms for Real time simulation of Algebraic Differential Equations systems (PARADE).
\end{itemize}

\section{Conferences Involvement}

\begin{itemize}
\item ROADEF 2017: Organizing committee member
\item CIE45: Organizing committee member
\item Sciences Incubator: Organizing committee member
\item CODIT'14: Organizing committee member
\item DASA16: Technical committee member
\item CloudNet16: Technical committee member 
\item CloudNet15: Technical committee member
\end{itemize}


